FreeSolo: Linear-time Sparse Attention with Zero-Shot Length Extrapolation

Linear-time sequence models typically store long-context information in a recurrent state. A fixed-size state limits how much information can be stored, while hybrid architectures that add full attention for better recall incur quadratic sequence cost. Alternatively, sparse attention with continued pretraining (CPT) can extend the effective context length. Generalization beyond the trained length remains challenging, however, and CPT can be costly. We introduce FreeSolo, a native sparse attention mechanism with a short-range sliding window branch and a long-range branch that selects keypoint cells for direct token attention. Its linear-time variant, FS-L, learns to prune the prefix before query-dependent selection through short CPT. FS-B searches balanced trees with $O(N\log^2 N)$ algorithmic cost including radix-sort construction. FreeSolo demonstrates better zero-shot length extrapolation than the baselines without long-context fine-tuning.

==> figures/causal_availability.tex <==
\node[small,anchor=west] at (.48,7.18) {Token sequence: $s=32$ tokens per cell};
\node[small,text=mypool] at (.14,6.60) {$\cdots$};
\foreach \slot in {0,...,7}{
  \pgfmathtruncatemacro{\rel}{\slot-8}
  \draw[draw=mypool,fill=mypool!18,line width=.45pt]
    ({.48+.76*\slot},6.35) rectangle ++(.70,.50);
  \node at ({.83+.76*\slot},6.60) {$c_{\rel}$};
}
\foreach \slot in {0,...,3}{
  \draw[draw=myquery!75,fill=myquery!10,line width=.45pt]
    ({6.56+.76*\slot},6.35) rectangle ++(.70,.50);
  \node[text=myquery] at ({6.91+.76*\slot},6.60) {$c_{\slot}$};
}
\draw[myblue,line width=.6pt] (8.29,6.85) -- (8.29,7.89);
\node[small,text=myquery,anchor=east] at (8.17,7.29) {$\vb q_i$};
\node[small,text=myquery] (startpos) at (6.53,7.20) {$0$};
\node[small,text=myquery] (endpos) at (9.57,7.20) {$128$};
\draw[queryflow] (startpos.south) -- (6.53,6.87);
\draw[queryflow] (endpos.south) -- (9.57,6.87);
\draw[decorate,decoration={brace,mirror,amplitude=2.5pt},mypool,line width=.4pt]
  (.48,6.22) -- (6.50,6.22)
  node[midway,below=2pt,small] {Full prefix $\mathcal C_i$};
\node[small,text=mypool] at (3.49,5.55)
  {All cells before this query block};
\draw[decorate,decoration={brace,mirror,amplitude=2.5pt},myquery,line width=.4pt]
  (6.56,6.22) -- (9.54,6.22)
  node[midway,below=2pt,small] {Query block: $B=128$};
\node[small,align=center,text=mypool] at (8.35,5.19)
  {Prefix boundary moves every query block\\[3pt]Fixed until the block ends};

\draw[mypool,line width=.65pt] (3.49,5.33) -- (3.49,5.15);
\draw[mypool,line width=.65pt] (2.05,5.15) -- (5.60,5.15);
\draw[poolflow] (2.05,5.15) -- (2.05,4.80);
\draw[poolflow] (5.60,5.15) -- (5.60,4.80);


==> figures/long_range_routers.tex <==
\node[title,text=myorange] at (.08,5.06) {Long range};
\node[panel,draw=mypool!70,fill=mypool!3,minimum width=3.20cm,
  minimum height=2.40cm] (densepool) at (2.05,3.60) {};
\node[panel,draw=mypool,fill=mypool!5,minimum width=3.20cm,
  minimum height=2.40cm] (sparsepool) at (5.60,3.60) {};
\node[small,text=mypool,font=\sffamily\bfseries\fontsize{8}{9.4}\selectfont]
  at (2.05,4.50) {FS};
\node[small,text=mypool,font=\sffamily\bfseries\fontsize{8}{9.4}\selectfont]
  at (5.60,4.50) {FS-L};
\node[small] at (2.05,4.10) {Keep the full prefix};
\node[small] at (5.60,4.10) {Prune per head};
\node[small,text=mypool] at (.77,3.38) {$\cdots$};
\node[small,text=mypool] at (4.32,3.38) {$\cdots$};
\foreach \slot in {0,...,11}{
  \draw[draw=mypool,fill=mypool!22,line width=.4pt]
    ({1.00+.21*\slot},3.25) rectangle ++(.17,.26);
  \draw[draw=black!28,fill=black!3,densely dashed,line width=.4pt]
    ({4.55+.21*\slot},3.25) rectangle ++(.17,.26);
}
\foreach \slot/\height in {0/.10,1/.31,2/.13,3/.07,4/.27,5/.11,6/.06,7/.29,8/.25,9/.12,10/.08,11/.10}{
  \fill[mypool!65] ({4.575+.21*\slot},3.58) rectangle ++(.12,\height);
}
\draw[mypool!80,densely dashed,line width=.45pt] (4.54,3.80) -- (7.04,3.80);
\foreach \slot in {1,4,7,8,10,11}{
  \draw[draw=mypool,fill=mypool!32,line width=.45pt]
    ({4.55+.21*\slot},3.25) rectangle ++(.17,.26);
}
\foreach \slot in {0,2,3,5,6,9}{
  \draw[black!35,line width=.45pt]
    ({4.57+.21*\slot},3.29) -- ++(.13,.18);
}
\node[small] at (2.05,2.92) {$\mathcal A_i=\mathcal C_i$};
\node[small,align=center] at (5.60,2.87)
  {$\mathcal A_i=\operatorname{TopP}_{c\in\mathcal C_i}(a_c)$\\[1pt]
   $\cup\,\operatorname{Recent}_W(\mathcal C_i)$};

\node[panel,draw=myorange!75,fill=myorange!3,minimum width=7.65cm,
  minimum height=2.10cm] (cellscore) at (4.30,1.15) {};
\node[small] at (4.30,1.88) {Cell scores with unrotated $\vb q_i,\bar{\vb k}_c$};
\node[small] at (4.30,1.15)
  {$r_{ic}=\textcolor{myquery}{\underbrace{
       \tfrac{\vb q_i^\top\bar{\vb k}_c}{\sqrt d}}_{\text{content match}}}
    +\textcolor{myorange}{\underbrace{\lambda_h a_c\,
       \erf\!\left(\tfrac{i-p_c}{2\sigma_h}\right)}
       _{\text{relative position bias}}},\quad c\in\mathcal A_i$};
\node[small] at (4.30,.42)
  {$\bar{\vb k}_c$: mean cell key;\quad $a_c=\max_{j\in\mathcal I_c}\norm{\vb k_j}_2$};
\draw[poolflow] (densepool.south) -- (2.05,2.20);
\draw[poolflow] (sparsepool.south) -- (5.60,2.20);

\node[panel,draw=myorange!80,fill=myorange!4,minimum width=4.05cm,
  minimum height=1.95cm] (select) at (10.425,1.00) {};
\node[small] at (10.425,1.62) {Top-$K$ per query and head};
\node[small,anchor=west] at (8.52,1.19) {FS};
\node[small,anchor=west] at (8.52,.83) {FS-L};
\foreach \yy in {1.06,.70}{
  \node[small,text=mypool] at (9.44,\yy+.13) {$\cdots$};
  \foreach \slot in {0,...,11}{
    \draw[draw=mypool,fill=mypool!22,line width=.4pt]
      ({9.68+.21*\slot},\yy) rectangle ++(.17,.26);
  }
}
\foreach \slot in {0,2,3,5,6,9}{
  \draw[draw=black!28,fill=black!3,densely dashed,line width=.4pt]
    ({9.68+.21*\slot},.70) rectangle ++(.17,.26);
  \draw[black!35,line width=.45pt]
    ({9.70+.21*\slot},.74) -- ++(.13,.18);
}
\foreach \yy in {1.06,.70}{
  \foreach \slot in {1,4,7,11}{
    \draw[draw=myorange,fill=myorange!38,line width=.45pt]
      ({9.68+.21*\slot},\yy) rectangle ++(.17,.26);
  }
}
\node[small] at (10.425,.39) {$\mathcal S_i$: tokens selected by $\vb q_i$};
\draw[globalflow] (cellscore.east) -- (cellscore.east -| select.west);
\node[panel,draw=myorange,fill=myorange!4,minimum width=3.60cm,
  minimum height=1.60cm,align=center,inner xsep=5pt,inner ysep=5pt]
  (lrread) at (9.90,3.25)
  {$\ell_{ij}=\tfrac{\vb q_i^\top\vb k_j}{\sqrt d},\quad j\in\mathcal S_i$\\[5pt]
   $\vb u_i^\top=\operatorname{softmax}(\boldsymbol\ell_{i,\mathcal S_i})^\top
     \vb V_{\mathcal S_i}$\\[5pt]
   $\vb o_i^{\mathrm{lr}}=\operatorname{RMSNorm}(\vb u_i)$};
\node[small,text=myorange] at (9.90,4.48) {NoPE readout, RMSNorm per head};
\draw[globalflow] (select.north) -- (select.north |- lrread.south);

\draw[draw=mypool,fill=mypool!22,line width=.45pt] (.55,-.32) rectangle ++(.19,.19);
\node[small,anchor=west] at (.81,-.225) {Prefix cell};
\draw[draw=myorange,fill=myorange!38,line width=.45pt] (3.05,-.32) rectangle ++(.19,.19);
\node[small,anchor=west] at (3.31,-.225) {Selected};
\draw[draw=black!28,fill=black!3,densely dashed,line width=.4pt]
  (5.10,-.32) rectangle ++(.19,.19);
\draw[black!35,line width=.45pt] (5.13,-.29) -- ++(.13,.13);
\node[small,anchor=west] at (5.36,-.225) {Pruned};
\draw[draw=myquery!75,fill=myquery!10,line width=.45pt]
  (7.03,-.32) rectangle ++(.19,.19);
\node[small,anchor=west] at (7.29,-.225) {Query block};

